Don't blame Dataset Shift! Shortcut Learning due to Gradients and Cross Entropy

Common explanations for shortcut learning assume that the shortcut improves prediction under the training distribution but not in the test distribution. Thus, models trained via the typical gradient-based optimization of cross-entropy, which we call default-ERM, utilize the shortcut. However, even when the stable feature determines the label in the training distribution and the shortcut does not provide any additional information, like in perception tasks, default-ERM still exhibits shortcut learning. Why are such solutions preferred when the loss for default-ERM can be driven to zero using the stable feature alone? By studying a linear perception task, we show that default-ERM's preference for maximizing the margin leads to models that depend more on the shortcut than the stable feature, even without overparameterization. This insight suggests that default-ERM's implicit inductive bias towards max-margin is unsuitable for perception tasks. Instead, we develop an inductive bias toward uniform margins and show that this bias guarantees dependence only on the perfect stable feature in the linear perception task. We develop loss functions that encourage uniform-margin solutions, called margin control (MARG-CTRL). MARG-CTRL mitigates shortcut learning on a variety of vision and language tasks, showing that better inductive biases can remove the need for expensive two-stage shortcut-mitigating methods in perception tasks.

==> sections/gradients.tex <==

\section{Function definitions and gradients}

\subsection{Log-loss}

\begin{align}
\ell(\theta^\top X, Y)  = - Y \log \sigma(\theta^\top X)
     - (1-Y)\log (1 - \sigma(\theta^\top X))
\end{align}


\begin{align}
   \nabla_\theta \ell(\ftheta(\mbx), \mby)) 
    & = -Y \frac{\nabla_\theta\sigma(\theta^\top X)}{\sigma(\theta^\top X)}
    % 
    + (1-Y)\times \frac{\nabla_\theta \sigma(\theta^\top X)}{(1 - \sigma(\theta^\top X))}
\\
& =
\left[- Y*(1 - \sigma(\theta^\top X))
  + (1-Y)\sigma(\theta^\top X)\right]X
\\
& =
\left[\sigma(\theta^\top X) - Y \right]X
\end{align}


\subsection{stiched log-loss}

\begin{align}
\ell(\theta^\top X, Y)  = - Y \log \sigma(\theta^\top X)
     - (1-Y)\log (1 - \sigma(\theta^\top X))
\end{align}



\subsection{Sigmoid-damping (label-dependent)}

The loss function is modified to damp the logits based on the label

\begin{align}
\text{logit}_\sigma(\theta,Y, X) = 
\theta^\top X   \times \left[1  - \left[Y*\sigma(\theta^\top X) + (1- Y) (1 - \sigma(\theta^\top X)\right]\right]))
\end{align}


\begin{align}
\nabla_\theta \ell(\text{logit}_\sigma, Y )& =
\left[\sigma(\theta^\top X) - Y \right] \nabla_\theta \text{logit}_\sigma(\theta,Y, X)
\\
&
    = \left[\sigma(\theta^\top X) - Y \right] 
    \bigg(
    X\times \left[1  - \left[Y*\sigma(\theta^\top X) + (1- Y) (1 - \sigma(\theta^\top X)\right]\right]))\bigg.
\\
& \quad \bigg. 
- \theta^\top X \times 
\left[Y * \sigma(\theta^\top X)(1 - \sigma(\theta^\top X))
- (1-Y)\sigma(\theta^\top X)(1-\sigma(\theta^\top X))\right] X
    \bigg)
\\
&
    = \left[\sigma(\theta^\top X) - Y \right] 
    \bigg(
    - \left[ (2Y - 1)\sigma(\theta^\top X) - Y )\right]))\bigg.
\\
& \quad \bigg. 
-
\left[2Y - 1\right] \sigma(\theta^\top X)(1-\sigma(\theta^\top X)) (\theta^\top X) 
    \bigg) X 
% \\
% & =  \left[\sigma(\theta^\top X) - Y \right] 
%  \left[2Y - 1\right]\sigma(\theta^\top X)
%  \bigg(-1 + \frac{Y}{\left[2Y - 1\right]\sigma(\theta^\top X)} - (1-\sigma(\theta^\top X)) (\theta^\top X) \bigg) X
\\
& =  \left[\sigma(\theta^\top X) - Y \right] 
 \left[2Y - 1\right]
 \bigg(\frac{Y}{\left[2Y - 1\right]} - \sigma(\theta^\top X) \left[1 + (1- \sigma(\theta^\top X)) (\theta^\top X)\right] \bigg) X
\\
& =  \left[\sigma(\theta^\top X) - Y \right] 
 \left[2Y - 1\right]
 \bigg(Y - \sigma(\theta^\top X) \left[1  +  (1-\sigma(\theta^\top X)) (\theta^\top X)\right] \bigg) X
\end{align}



\subsection{Norm constraint}

Output of the neural network is made to lie within $[-1,1]$ (can be multiplied by $M$ to get any range)

Given a representation $r(X)$ and last linear layer $\theta$, \normcons{} produces input to the log-loss as follows:
\begin{align}
   \texttt{logit}_\|(\theta, r(X)) = \frac{M*\theta^\top r(X)}{\|\theta\|\|r(X)\|}
\end{align}

Assuming $r(X)=X$ and is unit norm and $M=1$, the gradient of the modified logit w.r.t $\theta$ can be written as

\begin{align}
\nabla_\theta \texttt{logit}_\|(\theta, r(X)) & = -\nabla_\theta \left(\frac{\theta^\top}{\|\theta\|} X\right)
\\
						& =  \left(\frac{X}{\|\theta\|} - \frac{(\theta^\top X) \theta}{\|\theta\|^3}\right)
\\
					& =\left(\frac{\|\theta\|^2 \mathbf{I} - \theta\theta^\top}{\|\theta\|^3}\right) X
\\
					& =\left(\frac{\mathbf{I} - \frac{\theta\theta^\top}{\|\theta\|^2}}{\|\theta\|}\right) X
\end{align}

\subsection{Spectral decoupling}

Spectral decoupling modifies the loss function to penalize the norm of the logits.
For a penalization coefficient $\lambda$,
\begin{align}
\ell_{sd}(\theta^\top X, Y)  = \ell_{log-loss}(\theta^\top X, Y)  + \lambda |\theta^\top X|^2
\end{align}
% \section{Variants}

Gradients
\begin{align}
\nabla_\theta \ell_{sd}(\theta^\top X, Y)  = \left[\sigma(\theta^\top X) - Y + 
 2 \lambda (\theta^\top X)\right] X
\end{align}

\subsection{logistic link function with stitched bump}
Sigmoid rates with bump at $1$ to be put into the loss function 

Give $Y, f(X)$, log-loss (NLL with sigmoid links) is
\[\ell(Y, f(X)) = \log(1 + \exp(-(2Y-1)f(X)))\]

Denoting $v = (2Y-1)f(X)$, this loss function is 
\[\ell(Y, f(X)) = \log(1 + \exp(-v)\]

We modify $v$ before putting it into log-loss.
We make it so that for correctly classified samples with confidence $\sigma(1)$ (i.e. $v > 1$), the into to log-loss keeps decreasing, i.e. the loss goes up.
% 
\begin{align}
v^+ = 1[v \leq 1 ] v  - 1[v> 1 ]( 2 - v)
\end{align}

We can modify this to keep the bump anywhere: for a bump location $s$
\begin{align}
v^+ = 1[v \leq s] v  - 1[v> s ]( 2*s - v)
\end{align}

% \begin{align}
%     \frac{Y + \exp(l)(-2lY + l + 1 ) - \exp(2l)(Y-1)}{(\exp(2l) + 1)^2}
% \end{align}

%\subsection{The relationship between \normcons{} and \gls{sd}}\label{appsec:norm-sd}
%
%We first show the relationship between the solutions of logistic regression with \textsc{norm} and $\ell_2$-regularized logistic regression.
%Write the gradient for \textsc{nll} with \textsc{norm}: 
%%with $\left(\frac{w}{\|w\|}\right) = \frac{w^\top}{\|w\|}$,
%\begin{align}
%\nabla_w \ell\left(\frac{w^\top}{\|w\|} \mbx, \mby\right) & = - \left[1 - \sigma(\mby \left(\frac{w}{\|w\|}\right)^\top \mbx) \right] \mby \nabla_w \left(\frac{w^\top}{\|w\|} \mbx\right)
%%\\
%%						& =  - \left[1 - \sigma(\mby \left(\frac{w}{\|w\|}\right)^\top \mbx) \right] \mby \left(\frac{\mbx}{\|w\|} - \frac{(w^\top \mbx) w}{\|w\|^3}\right)
%%\\
%%					& =  - \left[1 - \sigma(\mby \left(\frac{w}{\|w\|}\right)^\top \mbx) \right] \mby \left(\frac{\|w\|^2 \mathbf{I} - ww^\top}{\|w\|^3}\right) \mbx
%%\\
%					& =  - \left[1 - \sigma(\mby \left(\frac{w}{\|w\|}\right)^\top \mbx) \right] \mby \left(\frac{\mathbf{I} - \frac{ww^\top}{\|w\|^2}}{\|w\|}\right) \mbx
%\end{align}
%
%Now, averaging across samples and setting the left hand to $0$, we get
%\begin{align}
%\left(\frac{\mathbf{I} - \frac{ww^\top}{\|w\|^2}}{\|w\|}\right)	\sum_i \left[1 - \sigma(\mby^i \left(\frac{w}{\|w\|}\right)^\top \mbx^i) \right] \mby^i \mbx^i = 0.
%\end{align}
%This is a matrix-vector product that can only be zero if the vector $\sum_i \left[1 - \sigma(\mby^i \left(\frac{w}{\|w\|}\right)^\top \mbx^i) \right] \mby^i \mbx^i$ lives in the null-space of matrix $\mathbf{I} - \frac{ww^\top}{\|w\|^2}$.
%The only unit vector in the null-space of $\mathbf{I} - \frac{ww^\top}{\|w\|^2}$ is $\frac{w}{\|w\|}$.
%Thus, the solution to logistic with the \textsc{norm} constraint is 
%	\[w^*_{\textsc{norm}} \propto \sum_i \left[1 - \sigma(\mby^i \left(\frac{w^*_{\textsc{norm}} }{\|w^*_{\textsc{norm}} \|}\right)^\top \mbx^i) \right] \mby^i \mbx^i .\]
%
%Now, notice the gradient for logistic regression such that $\ell_2$ penalty on $w$:
%\begin{align}
%	\nabla_w \ell\left(\frac{w^\top}{\|w\|} \mbx, \mby\right) + \lambda \|w\|^2 & = - \left[1 - \sigma(\mby w^\top \mbx) \right] \mby  \nabla_w w^\top\mbx +  \lambda \nabla_w w^\top w.
%\end{align}
%Setting the average of this over $i$ to 0, we get that 
%\begin{align}
%		w^*_{\ell_2} \propto \sum_i \left[1 - \sigma(\mby^i (w^*_{\ell_2})^\top \mbx^i) \right] \mby^i \mbx^i.
%\end{align}
%Choose $\lambda$ such that $\|w^*_{\ell_2}\|=1$ so we have $\nicefrac{w^*_{\ell_2}}{\|w^*_{\ell_2}\|}=w^*_{\ell_2}$. Assuming uniqueness of solutions for $w^*_{\ell_2}, w^*_{\textsc{norm}}$, we have $w^*_{\ell_2}= w^*_{\textsc{norm}}$ because they satisfy the same equation with respect to the data.
%%because $\frac{w^*_{\ell_2}}{\|w^*_{\ell_2}\|} = $
%
%Now, if $\forall i, \|\mbx^i\|=1$, then for any $w$ and the same $\lambda$ as the penalizing coefficient, the value of the $\ell_2$-regularized logistic regression upper bounds the spectral decoupling objective.
%To see this, the log-likelihood is the same because $w$ is fixed, and note that as the penalty in spectral decoupling is bounded as follows when $\|\mbx^i\|=1$:
%\[\lambda (w^\top x)^2 \leq \lambda \|w\|^2\|x\|^2 = \lambda \|w\|^2.\]
%
%




==> sections/noise_bias.tex <==
\begin{thm}
Let $\mby, \mbz$ be rademacher random variables such that $p(\mby=\mbz) = \rho>0$.
For a positive constant $B$, let the covariates be $\mbx = [\mby, B \mbz, \mbeps]$ such that the following condition holds:
\[\forall i, j \quad \|\mbeps^i\| = \|\mbeps^j\|= \sqrt{\Gamma}, \quad \mbeps^i \perp \mbeps^j.\]
Let parameters $\theta=[w_y, w^\prime_z, v]$ parameterize a linear function: 
\begin{align}
	\ftheta(\mbx) = w_y \mby + B w^\prime_z \mbz + v^\top\mbeps.
\end{align}
Consider training the the model $\ftheta(\mbx)$ on $n$ samples from the DGP above using log-loss with gradient descent with an infinitesimal step size; so, each of $w_y, w^\prime_z, v$ have a gradient flow associated with them.
Letting $w_z=B w^\prime_z$, the solution paths for the parameters $w_y(t), w_z(t)$ are defined by the following coupled ODEs:
%
\begin{align}
	\dot{w_y}(t)
%	& =  \frac{\rho}{1 + \exp(w_y(t) + w_z(t)   + \frac{\Gamma}{2n\rho} (w_y(t) + w_z(t)) )}  + \frac{1-\rho}{1 + \exp(w_y(t) - w_z(t) + \frac{\Gamma}{2n(1-\rho)} ( w_y(t) - w_z(t)))}
%\\ 
	& =  \frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) + w_z(t)) \right]}  + \frac{1-\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t) - w_z(t))\right]}
\\
\dot{w_z}(t)
%	&  =  \left[ \frac{\rho}{1 + \exp(w_y(t) + w_z(t) +  \frac{\Gamma}{2n\rho} (w_y(t) + w_z(t)) )} - \frac{1-\rho}{1 + \exp(w_y(t) - w_z(t)  + \frac{\Gamma}{2n(1-\rho)} (w_y(t) - w_z(t)))}  \right]
%\\ 
	& =  \frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) + w_z(t)) \right]}  - \frac{1-\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t) - w_z(t))\right]}
\end{align}
	
\end{thm}


\begin{proof}
%\newcommand{\dot}[1]{\dot{#1}}
We define the gradient flows for this model on $n$ samples for any $w\in \{w_y, Bw^\prime_z, v\}$, and $\mby^i\mbeps^i = \gamma^i$.
We define the gradient flow for $w_z = B w^\prime_z$  instead of just $w^\prime_z$ to make math simpler.
%
Suppressing the dependence on $t$ on the right side
\begin{align*}
	\dot{w}(t) &= - \frac{1}{n}\sum_i \nabla_{w} \log (1 + \exp(-\mby^i \ftheta(\mbx^i)) )
\\
	& = - \frac{1}{n}\sum_i  \frac{-\exp(-\mby^i \ftheta(\mbx^i))}{1 + \exp(-\mby^i \ftheta(\mbx^i))} \nabla_w (w_y + w_z \mby^i \mbz^i  + v^\top \mby^i \mbeps^i)
\\
	& =  \frac{1}{n}\sum_i  \frac{1}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \mby^i \mbeps^i)} \nabla_w (w_y + w_z \mby^i \mbz^i  + v^\top \mby^i \mbeps^i)
\\
	& = \frac{1}{n}\sum_i  \frac{1}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)} \nabla_w (w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)
\end{align*}



Then,
\begin{align*}
	\dot{w_y}(t)
	& = \frac{1}{n}\sum_i  \frac{1}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)}
\\
\dot{w_z}(t)
	& =  \frac{1}{n}\sum_i  \frac{ \mby^i \mbz^i}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)} 
\\
\dot{v}(t)
	& =  \frac{1}{n}\sum_i  \frac{\gamma^i}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)} 
\end{align*}



Now, let us look at flow for the part of $\ftheta(\mbx^i)$ that comes from noise:
\begin{align}
\dot{v}(t)^\top \gamma^j
	& =  \frac{1}{n}\sum_i \frac{(\gamma^i)^\top \gamma^j}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)} 
\\
   & =  \frac{\|\gamma^j\|^2}{n\left(1 + \exp(w_y + w_z \mby^j \mbz^j  + v^\top \gamma^j)\right)} 
\\
%	& = \frac{\Gamma}{1 + \exp(w_y + B w_z \mby^j \mbz^j  + v^\top \gamma^j)}
\\
	& = \frac{\Gamma}{n}\frac{1}{1 + \exp(w_y + w_z \mby^j \mbz^j  + v^\top \gamma^j)}
\end{align}

Define $\eta(t)_j = v(t)^\top \gamma^j $ and  noting that $\nabla_t (v(t)^\top \gamma^j) = \dot{v(t)}^\top \gamma^j$, we can rewrite the the flow above as,


\begin{align}
\frac{d \eta(t)_j}{dt}
	& =  \frac{\Gamma}{n}\frac{1}{1 + \exp(w_y + w_z \mby^j \mbz^j  + \eta(t)_j)}
\\ 
& = \begin{cases}
	 \frac{\Gamma}{n}\frac{1}{1 + \exp(w_y + w_z  + \eta(t)_j)} \qquad \forall j \in S
	 \\ \frac{\Gamma}{n}\frac{1}{1 + \exp(w_y -  w_z + \eta(t)_j)} \qquad \forall j \not\in S
\end{cases}
\end{align}
Assume that $\eta(t=0)_j = 0$ and we see that $\frac{d \eta(t)_j}{dt}$ has the same differential equation and initial condition for all $j\in S$.
The same is true for $j\not\in S$.
%
Then, we can define
\begin{align}
	\eta(t)_j  & = v(t)^\top \gamma^j  = u(t) \qquad \forall j \in S 
\\
	\eta(t)_j  & = v(t)^\top \gamma^j  = v(t) \qquad \forall j  \not\in S 
\end{align}





With this new expression, let's rewrite the flows for $w_y, w_z, u, v$ using sets $S = \{i: \mby^i = \mbz^i\}$ and $S^c = \{i :  \mby^i \not= \mbz^i\}$: noting that $ \forall i\in S \mby^i\mbz^i = 1$  and $\forall i \not\in S \mby^i\mbz^i=-1$,
%
\begin{align}
	\dot{w_y}(t)
	& = \frac{1}{n}\left[\sum_{i\in S}  \frac{1}{1 + \exp(w_y +  w_z \mby^i \mbz^i  + v^\top \gamma^i)}  + \sum_{i\not\in S}\frac{1}{1 + \exp(w_y +  w_z \mby^i \mbz^i  + v^\top \gamma^i)}\right]
\\
& = \frac{1}{n}\left[\sum_{i\in S}  \frac{1}{1 + \exp(w_y +  w_z   + v^\top \gamma^i)}  + \sum_{i\not\in S}\frac{1}{1 + \exp(w_y - w_z + v^\top \gamma^i)}\right]
\\
& = \frac{1}{n}\left[\sum_{i\in S}  \frac{1}{1 + \exp(w_y +  w_z   + u)}  + \sum_{i\not\in S}\frac{1}{1 + \exp(w_y -  w_z + v)}\right]
\\
& =  \frac{\rho}{1 + \exp(w_y + w_z   + u)}  + \frac{1-\rho}{1 + \exp(w_y - w_z + v)}
\\
\dot{w_z}(t)
	& =  \frac{1}{n}\left[\sum_{i\in S}  \frac{ \mby^i \mbz^i}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)} + \sum_{i\not\in S} \frac{ \mby^i \mbz^i}{1 + \exp(w_y + w_z \mby^i \mbz^i  + v^\top \gamma^i)}  \right]
\\
	& =  \frac{1}{n}\left[\sum_{i\in S}  \frac{1}{1 + \exp(w_y + w_z + v^\top \gamma^i)} - \sum_{i\not\in S} \frac{1}{1 + \exp(w_y - w_z  + v^\top \gamma^i)}  \right]
\\
	& =  \frac{1}{n}\left[\sum_{i\in S}  \frac{1}{1 + \exp(w_y + w_z +  u)} - \sum_{i\not\in S} \frac{1}{1 + \exp(w_y - w_z  + v)}  \right]
\\
	& =  \left[ \frac{\rho}{1 + \exp(w_y + w_z +  u)} - \frac{1-\rho}{1 + \exp(w_y - w_z  + v)}  \right]
\\\\
\dot{u(t)}
	& = 
	 \frac{\Gamma}{n}\frac{1}{1 + \exp(w_y + w_z  + u)} \\
	& = \frac{\Gamma}{n}\left(\frac{\dot{ w_y(t)} + \dot{w_z(t)}}{2 \rho}\right) 
\\
\dot{v(t)} & = 
	 	\frac{\Gamma}{n}\frac{1}{1 + \exp(w_y -  w_z + v)}
\\
	& = \frac{\Gamma}{n}\left(\frac{\dot{ w_y(t)} -  \dot{w_z(t)}}{2(1 - \rho)}\right) 
\end{align}
The last two expressions mean that we can write $u(t), v(t)$ as follows for any $t$
\begin{align}
u(t) = \frac{\Gamma}{2n\rho} (w_y(t) + w_z(t))
	\qquad \qquad \qquad v(t) = \frac{\Gamma}{2n(1-\rho)} (w_y(t) - w_z(t))
\end{align}


Finally, we can use the expressions for $u(t), v(t)$ to reduce the system for $w_y, w_v, v$ into the only two coupled gradient flows:

\begin{align}
	\dot{w_y}(t)
	& =  \frac{\rho}{1 + \exp(w_y(t) + w_z(t)   + \frac{\Gamma}{2n\rho} (w_y(t) + w_z(t)) )}  + \frac{1-\rho}{1 + \exp(w_y(t) - w_z(t) + \frac{\Gamma}{2n(1-\rho)} ( w_y(t) - w_z(t)))}
\\ 
	& =  \frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) + w_z(t)) \right]}  + \frac{1-\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t) - w_z(t))\right]}
\\
\dot{w_z}(t)
	&  =  \left[ \frac{\rho}{1 + \exp(w_y(t) + w_z(t) +  \frac{\Gamma}{2n\rho} (w_y(t) + w_z(t)) )} - \frac{1-\rho}{1 + \exp(w_y(t) - w_z(t)  + \frac{\Gamma}{2n(1-\rho)} (w_y(t) - w_z(t)))}  \right]
\\ 
	& =  \frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) + w_z(t)) \right]}  - \frac{1-\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t) - w_z(t))\right]}
\end{align}

\end{proof}

\begin{thm}
Solving the gradient flows. TODO
\end{thm}
\begin{proof}
Now, we can make this coupled system into two disparate ODEs, one for $\dot{w_y}(t) + \dot{w_z}(t)$ and one for $\dot{w_y}(t) - \dot{w_z}(t)$:
\begin{align}
	\dot{w_y}(t) + \dot{w_z}(t)
			& =  \frac{2\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) + w_z(t)) \right]}
\\ 
	\dot{w_y}(t) - \dot{w_z}(t)
			&  =  \frac{2(1-\rho)}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t) - w_z(t))\right]} 
\end{align}


\section{Needed theorems}

\begin{thm}
    Assume \gls{dgp} 
\end{thm}

%By pulling the denominator on the RHS to the LHS, we get the following equations:
%\begin{align}
%	{w_y}(t) + {w_z}(t) + \frac{\exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) + w_z(t)) \right] - 1 }{\left(1 + \frac{\Gamma}{2n\rho}\right)} 
%			& =  2\rho t 
%%\\
%%	\text{Rearranging:} \qquad 
%%%	\\
%%		\left(1 + \frac{\Gamma}{2n\rho}\right)\left({w_y}(t) + {w_z}(t)\right)+ {\exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) + w_z(t)) \right]}			& =  2\rho t \left(1 + \frac{\Gamma}{2n\rho}\right) + 1
%\\
%%\\\\\\
%{w_y}(t) - {w_z}(t) + \frac{\exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t) - w_z(t))\right] - 1}{\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}
%			&  =  2(1-\rho) t
%%\\
%%	\text{Rearranging:} \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad
%%	\\
%%\left( 1 + \frac{\Gamma}{2n(1-\rho)}\right)
%%\left({w_y}(t) - {w_z}(t)\right)
%% + {\exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t) - w_z(t))\right]}
%%			&  =  2(1-\rho) t\left( 1 + \frac{\Gamma}{2n(1-\rho)}\right) + 1
%\end{align}
%
%
%Adding the two equations, we get
%\begin{align}
%	w_y(t) + 2\sqrt{\frac{\exp{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right) w_y(t) + \left(\frac{\Gamma}{2 n\rho} - \frac{\Gamma}{2n(1-\rho)}\right) w_z(t)}}{\left(1 + \frac{\Gamma}{2n\rho}\right)\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}}
%\leq 
%		2t + \frac{1}{\left(1 + \frac{\Gamma}{2n\rho}\right)} + \frac{1}{\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}
%\end{align}
%
%Next, we simplify the numerator inside the square-root.
%Now, $w_z(t)\geq 0$ because when $w_z(t) = 0$, we have $\dot{w_z}(t) > 0$, see \cref{proof:pos-wz}.
%Further $\frac{\Gamma}{2 n\rho} - \frac{\Gamma}{2n(1-\rho)} > 0$ because $\rho > 1-\rho$.
%Thus, 
%\[\exp\left[{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right) w_y(t) + \left(\frac{\Gamma}{2 n\rho} - \frac{\Gamma}{2n(1-\rho)}\right) w_z(t)}\right] \geq  \exp\left[{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right) w_y(t)}\right].\]
%
%Further, noting that $\dot{w_y}(t) > 0$, which means $w_y(t) > 0$, and we get
%\begin{align}
%	&w_y(t) + 2\sqrt{\frac{\exp{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right) w_y(t)}}{\left(1 + \frac{\Gamma}{2n\rho}\right)\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}}
% \leq 
%		2t + \frac{1}{\left(1 + \frac{\Gamma}{2n\rho}\right)} + \frac{1}{\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}
%\\
%\implies  &
%w_y(t) + 2\sqrt{\frac{\exp{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right) w_y(t)}}{\left(1 + \frac{\Gamma}{2n\rho}\right)\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}}
% \leq 
%		2t + \frac{1}{\left(1 + \frac{\Gamma}{2n\rho}\right)} + \frac{1}{\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}
%\\
%\implies  &
%2\sqrt{\frac{\exp{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right) w_y(t)}}{\left(1 + \frac{\Gamma}{2n\rho}\right)\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}}
% \leq 
%		2t + \frac{1}{\left(1 + \frac{\Gamma}{2n\rho}\right)} + \frac{1}{\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}
%\\
%\implies  &
%{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right) w_y(t)} 
% - \frac{1}{2}\log \left(1 + \frac{\Gamma}{2n\rho}\right)\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)
% \leq 
%		\log (t + 1)
%\\
%\implies  &
%{ w_y(t)} 
%\leq 
%		\frac{\log (t + 1) + \frac{1}{2}\log \left(1 + \frac{\Gamma}{2n\rho}\right)\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)}{\left(2 + \frac{\Gamma}{2 n\rho} + \frac{\Gamma}{2n(1-\rho)}\right)}
%\end{align}
%
%
%
%
%
%
%\subsubsection{Showing the the spurious coefficient is non-negative}\label{proof:pos-wz}
%\begin{align}
%	\dot{w_z}(t) & = \frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) ) \right]}  - \frac{1-\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t))\right]}	
%%\\
%%	& \geq 
%%			\frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) ) \right]}  - \frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n(1-\rho)}\right)( w_y(t))\right]} \qquad \qquad \{ 1 - \rho < \rho
%%
%\\
%	& \geq 
%			\frac{\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) ) \right]}  - \frac{1-\rho}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho}\right)( w_y(t))\right]} \qquad \qquad \{ 1 - \rho < \rho
%\\
%	& \geq 
%			\frac{2\rho-1}{1 + \exp\left[\left(1 + \frac{\Gamma}{2n\rho} \right)(w_y(t) ) \right]}
%\\
%	& > 0
%\end{align}
%
%
%
%


\end{proof}





==> sections/old_dual_part_proof.tex <==

We maximize over $\nu$ first.
The derivative of the quadratic term is $2 \nu \|c^2\| + 2c^\top X^\top \lambda$ which is 0 when $\nu = \frac{-c^\top X^\top \lambda}{\|c\|^2}$.
% Substituting this value back in the problem above gives the term
% \begin{align}
%     -\frac{1}{4}\left\|-\frac{c c^\top}{\|c\|^2} X^\top \lambda + X^\top\lambda\right\|^2  +  \frac{1}{2}  \ind^\top \lambda =  -\frac{1}{4}\left\|\left(\mathbb{I} - \frac{c c^\top}{\|c\|^2}\right) X^\top \lambda\right\|^2   +  \frac{1}{2}  \ind^\top \lambda 
% \end{align}

Here we need $\nu \geq 0$ and we choose $\gamma$ to get $-c^\top X^\top \lambda \geq 0.$
We now specify a $\lambda$ such that $-c^\top X^\top w=0$, i.e. optimal $\nu=0$.
% 
% 
% We now specify a setting of where $\nu=0$, to achieve which we choose a $\lambda$ such that $c \perp X^\top \lambda=0$.
Let $k=|S_{min}|$.
% 
For a set $U\subset [n]$, we let $\lambda_i=\frac{\alpha}{|U|}$ for $i\in U$ and $0$ otherwise.
Specifically $U = S_{min} \cup \{\frac{2k}{(1- \nicefrac{1}{B^2})}-k \text{ samples from } S_{maj}\}$.
% We do this by letting $\lambda_i= \alpha$ for $i\in S_{min}$ and $\frac{2k}{(1- \nicefrac{1}{B^2})}-k$ samples from $S_{maj}$, and $0$ otherwise.
Note that the second element of $\mbx_i$ is $-B$ if $i\in S_{min}$ and $B$ if $i\in S_{maj}$.
So adding $k$ rows from $S_{min}$ and $k$ rows from $S_{maj}$ cancels out the $B$s and, so in $B$ is accumulated ${|U| - 2k}$ times.
Then,
\[X^\top \lambda = \left[\alpha, \alpha * \frac{|U|-2k}{|U|}, \frac{\alpha}{|U|} \sum_{i\in U}\mbdelta_{i} \right]= \left[\alpha, B\frac{\alpha}{B^2}, \frac{\alpha}{|U|} \sum_{i\in U}\mbdelta_{i}\right],\]
where we used the factsa
\[|U| = \frac{2k}{1 - \nicefrac{1}{B^2}} \qquad \qquad \frac{|U| - 2k}{|U|} = \frac{ \frac{2k}{1 - \nicefrac{1}{B^2}} - 2k}{ \frac{2k}{1 - \nicefrac{1}{B^2}}} =  \frac{ \frac{\nicefrac{2k}{B^2}}{1 - \nicefrac{1}{B^2}}}{ \frac{2k}{1 - \nicefrac{1}{B^2}}} = \frac{1}{B^2}.\]
Then
\[c^\top X^\top \lambda = [1, -B] [\alpha, \frac{\alpha}{B} ]^\top = 0.\]

Thus, we now evaluate the objective value, having set $\nu=0$.
We establish two facts first :
\begin{enumerate}
    \item 
            As $\lambda$ has $\frac{\alpha}{|U|}$ on $|U|$ elements and $0$ otherwise, $\lambda^\top \ind  = {\alpha}$
\item The term $\frac{1}{|U|}\sum_{i\in U}\mbdelta_{i}$ is a mean of $|U|$ standard normal vectors, and thus has the same distribution as a standard norm multiplied by $\frac{1}{\sqrt{|U}}$. Then, with probability at least $1-\exp(-ct^2/2)$ (theorem 3.1.1, Versheynin HDP book),
\[\left\|\frac{1}{|U|}\sum_{i\in U}\mbdelta_{i}\right\| \leq \frac{1}{\sqrt{|U|}}\left(\sqrt{d} + t\right).\]
\end{enumerate}

Setting $\nu=0$,
\begin{align}
   \|c\nu + X^\top\lambda\|^2  =\|X^\top\lambda\|^2  & = 
\left\| \left[\alpha, \frac{\alpha}{B}, \frac{\alpha}{|U|} \sum_{i\in U}\mbdelta_{i}\right] \right\|^2
\\
    & = \alpha^2\left\|\left[1, \frac{1}{B}, \frac{1}{|U|} \sum_{i\in U}\mbdelta_{i}\right]\right\|
    % \left(1 + \frac{1}{B^2} + \left\|\frac{1}{|U|} \sum_{i\in U}\mbdelta_{i}\right\|^2\right) + \frac{\alpha}{2}
% \\
%     & \leq \alpha^2
%     (1 + \frac{1}{B^2} + \left(\frac{\sqrt{d} + t}{\sqrt{|U|}}\right)^2)
% \\
%     & \geq \frac{1}{2}\left(\alpha- \frac{\alpha^2}{2}
%     (1 + \frac{1}{B^2} +\left(\frac{\sqrt{d} + t}{\sqrt{|U|}}\right)^2)\right) 
    \label{eq:lb-unopt}
\end{align}


% Letting $b=\frac{1}{2}
%     (1 + \frac{1}{B^2} + \left(\frac{\sqrt{d} + t}{\sqrt{|U|}}\right)^2)$,
% \cref{eq:lb-unopt} is a quadratic function of the form $-ba^2 + a$ which is maximized by setting $a = \frac{1}{2b}$, achieving a value of $\frac{1}{4b}$.
% 
% \begin{align}
%     -\frac{1}{4}\|X^\top\lambda\|^2  + \frac{1}{2}\lambda^\top \ind & = - \frac{1}{4}\left\| \left[\alpha, \frac{\alpha}{B}, \frac{\alpha}{|U|} \sum_{i\in U}\mbdelta_{i}\right] \right\|^2 + \frac{\alpha}{2}
% \\
%     & = - \frac{\alpha^2}{4}\left(1 + \frac{1}{B^2} + \left\|\frac{1}{|U|} \sum_{i\in U}\mbdelta_{i}\right\|^2\right) + \frac{\alpha}{2}
% \\
%     & \geq \frac{\alpha}{2} - \frac{\alpha^2}{4}
%     (1 + \frac{1}{B^2} + \left(\frac{\sqrt{d} + t}{\sqrt{|U|}}\right)^2)
% \\
%     & \geq \frac{1}{2}\left(\alpha- \frac{\alpha^2}{2}
%     (1 + \frac{1}{B^2} +\left(\frac{\sqrt{d} + t}{\sqrt{|U|}}\right)^2)\right) 
%     \label{eq:lb-unopt}
% \end{align}
% Letting $b=\frac{1}{2}
%     (1 + \frac{1}{B^2} + \left(\frac{\sqrt{d} + t}{\sqrt{|U|}}\right)^2)$,
% \cref{eq:lb-unopt} is a quadratic function of the form $-ba^2 + a$ which is maximized by setting $a = \frac{1}{2b}$, achieving a value of $\frac{1}{4b}$.
% % 
% 
% Setting $t=\sqrt{\theta^2 d}$, the bound simplifies $\left(\frac{\sqrt{d} + t}{\sqrt{|U|}}\right)^2 = \frac{(1+\theta)^2d}{|U|}$.
% \footnote{CHOICE: $t=\sqrt{\theta^2 d}$ which makes the chances of the bound not happening exponentially small in $\theta^2 d$}.
% So the lower bound we started out to find is
% \begin{align}
%     C_c 
% & = \frac{1}{2}\left(\frac{1}{4\left[\frac{1}{2}\left(1 + \frac{1}{B^2} + \frac{(1+\theta)^2d}{|U|} \right)\right]}\right) 
% \\
% & 
%     = 
%     \frac{1}{4\left({\left[\left(1 + \frac{1}{B^2} + \frac{(1+\theta)^2d}{2k}\left(1 - \frac{1}{B^2}\right)\right)\right]}\right)}
% \\
% & 
%     = 
%     \frac{B^2}{4\left(B^2 + 1 + \frac{(1+\theta)^2d}{2k}\left(B^2 - 1\right)\right)}
% \end{align}


% \hl{TODO: change this to not have lower bound on $k$.}

% % Here, let $k \geq  \frac{\theta_1}{2} \sqrt{d}$.
% % Choosing $\frac{(1+\theta)^2}{\theta_1} = \sqrt{2}$,
% Setting $\frac{(1+\theta)^2}{2} = \sqrt{1}$, and noting that $d > k^2$
% \begin{align}
%     C_c & 
%     = 
%     \frac{B^2}{4\left(B^2 + 1 + \frac{(1+\theta)^2d}{2k}\left(B^2 - 1\right)\right)}
% % \\
%     % & \geq 
%     % \frac{B^2}{4\left(B^2 + 1 + \frac{(1+\theta)^2}{\theta_1} \frac{d}{    \sqrt{d}}\left(B^2 - 1\right)\right)}
% \\
%     & =     \frac{B^2}{4\left(B^2 + 1 + \frac{d}{k}\left(B^2 - 1\right)\right)}
% % \\
%     % & =     \frac{B^2}{4\left(B^2 + \sqrt{2d}B^2 + 1 - \sqrt{2d}\right)}
% \\
%     & \geq  \frac{B^2}{4\left(B^2 + \frac{d}{k}B^2\right)} \qquad \qquad \{\frac{d}{k} > 1 \}
% \\
%     & 
%     = \frac{1}{4(1 + \frac{d}{k})}.
% % \\
% %     &
% %     \geq  \frac{k}{8d}    \qquad \qquad  \qquad  \qquad  \qquad \{\frac{d}{k} > 1 \}
% \end{align}

% TODO: subscripts can be confusing here; what are they indexing?



% \paragraph{Concluding the proof}


% Here, we show that for large enough $B$, it holds that $C_s < C_c$.
% Then, the max-margin solution will achieve lower norm by violating the constraint $w_y \geq B w_z $.
% Thus, $\frac{B w_z^*}{w^*_y } > 1.$
% We need to compare these two:
% \begin{align}
%     C_s &
% = \frac{k}{\eta^2d}\left[\left(\frac{ 1 + \frac{\eta\sqrt{d}}{\sqrt{k}}}{B}\right)^2 + 1\right]
% % \\
% % & 
% % < \frac{1}{\eta^2\sqrt{d}}2
% % \\
% % &
% % = \frac{k}{8d}
% \\
% & \text{and}
% \\
% C_c & \geq \frac{1}{4(1 + \frac{d}{k})}.
% \end{align}


% \hl{This requires $\eta \geq \sqrt{4(1 + \frac{k}{d})} > 1$ but $\eta < \frac{1}{3}$ by definition.}


TODO: the following might be the right to do things.


==> sections/old_paper.tex <==

\section{Catastrophic remembering: fast features get preserved}


\subsection{Setup}
We focus on classification tasks with $\mby \in \{-1, 1\}$ as the label, and $\mbx$ as the covariates.
We let $\ptr$ and $\pte$ be train and test distributions respectively.
% Unless other mentioned $\ptr = \pte$.
TODO: more details
TODO: define balancing, spectral decoupling etc.

\subsection{Understanding shortcut learning on preservation tasks}
Much work on explaining and tackling shortcut learning focuses on cases where the shortcut and the invariant features are both imperfect \citep{sagawa2020investigation,arjovsky2019invariant,krueger2020out}(cite more). 
In this cases, in the limit of infinite data, \gls{erm} achieves optimal performance only when relying on both features.
However, many common \gls{ood} tasks where shortcut learning in \gls{erm} is evaluated, are perception tasks, where the invariant 
% \footnote{Semantics are features that humans use to classify, and have invariant relationships with the label across training and test data.} 
% 
feature is often a perfect predictor.
For example, in image recognition tasks CelebA and Waterbirds \citep{sagawa2019distributionally}, hair color and the shape of the bird respectively determine the label.

When a perfect predictor exists in $\mbx$, \gls{erm} with a sufficiently flexible model class will rely only on the perfect feature in the limit of infinite data; this is because for a perfect feature $\perf(\mbx)$ that determines the label, $\ptr(\mby\g \mbx) = \ptr(\mby\g \perf(\mbx))$.
Then, as perfect invariant features are invariant by definition $\ptr(\mby \g \perf(\mbx)) = \pte(\mby \g \perf(\mbx))$ and as \gls{erm}-models learn the training data conditional $\ptr(\mby\g \mbx)$, they are optimal on test.
However, methods that mitigate shortcut learning in finite-sample (CITE), are also typically derived in the same infinite sample regime where \gls{erm} is also expected to work.
% 
% 
% 

Therefore on perception tasks, a finite-sample phenomenon must explain both the methods that mitigate shortcut learning and why \gls{erm} falls prey to shortcuts.
However, work that aims to explain shortcut learning \citep{sagawa2020investigation,shah2020pitfalls,pezeshki2021gradient,nagarajan2020understanding} does not provide a single unifying finite-sample phenomenon.
% explains shortcut learning as a consequence of gradient-based training of neural networks.
% using 1) simplicity bias, 2) 
% 
% 
Specifically, the following questions arise:
% 
% about flexible neural networks trained on perception tasks that we provide an answer for using a single mechanism.
% \textit{the race between learning different features}.
% 
% 
% We focus on the high-level points made by related work.
% 
\begin{enumerate}
    % \item Why do neural networks prefer imperfect predictors over perfect predictors?
    % 
    
    \item Even if an imperfect feature is a simpler function of the covariates and gets picked up early during training in \gls{erm} (as suggested by \citep{shah2020pitfalls,nakkiran2019sgd}), why would a perfect feature not be learned later in training?
    
    \item When and where do existing methods that mitigate shortcut learning (balancing) and simplicity bias (spectral decoupling) help, while \gls{erm} fails? 
    % 
    While Sagawa provide one explanation for balanced-\gls{erm} via subsampling, they reason only about solutions, but not solution paths, and therefore do not explain spectral decoupling.
    In contrast, \citep{pezeshki2021gradient} reason about solution paths and derive spectral decoupling in the idealized NTK regime, their theory only holds when each feature appears in only a single sample; thus, their theory cannot explain why balancing helps, unlike \gls{erm}?
    % \citep{sagawa2019distributionally} explain this in 
    
    % \item Where do methods like spectral decoupling help? 
    % \citet{sagawa2020investigation} explain 
    
    \item What role does overparameterization play? While \citep{nagarajan2020understanding} study perfect invariant features and imperfect shortcuts and allow for overparameterization in their setup, they do not study its role.
    % 
    
    % TODO: we could probably explain the increasing norms phenomenon, at least in the linear case; more (orthogonal) samples to memorize, more norm because norms of sums of orthogonal vectors are sums of norms of each.
\end{enumerate}


We answer these questions by reasoning about which features models pick up first during training. 
That is, we study a mechanism behind shortcut learning in perception tasks that emerges out of \textit{the learning race between different features}.
We first give an intuitive explanation of why quickly learnable features are often preserved in gradient-based training of overparameterized models; we call this \textit{preservation bias}, and study it empirically.


\paragraph{An intuitive presentation of how learning preservation bias.}
% 
Imagine there exist two informative features --- a perfect invariant $\perf(\mbx) = \mby$, and an imperfect shortcut $\sho(\mbx) \in \{-1,1\}$ that equals $\mby$ w.p. $\rho$, and non-informative noise features $n(\mbx)$.
% 
We start by looking at the per-sample gradient of the log-loss $\ell(\ftheta(\mbx), \mby)) = \log \left[1 + \exp(-\mby \ftheta(\mbx))\right]$ with respect to the model parameters $\theta$: with $\sigma(a) = \nicefrac{1}{1 + \exp(-a)}$,
\[\nabla_\theta \ell(\ftheta(\mbx), \mby)) = -\frac{\exp(-\mby \ftheta(\mbx))}{1 + \exp(-\mby \ftheta(\mbx))} \nabla_\theta f_\theta(\mbx) = - \left[1 - \sigma(\mby \ftheta(\mbx)) \right]\nabla_\theta f_\theta(\mbx).\]
% 
% 
The magnitude of the gradient from each sample is modulated by how confidently correct the prediction on that sample is; as $\mby \ftheta(\mbx)$ gets larger, $\nabla_\theta f_\theta(\mbx)$ gets smaller.
% 

Now, assume that the shortcut won the learning race over the invariant feature, due to, for example, the simplicity bias \citep{shah2020pitfalls}.
For illustration, consider that the model learns to rely only on the shortcut $\sho(\mbx)$ on every sample.
Then, in the training data, the $(1 - \sigma(\cdot))$ term in the gradient approaches $0$ for samples that are correctly classified by the shortcut; call this the \textit{shortcut-classified} subset where $\sho(\mbx)=\mby$.

% As this $(1 - \sigma(\cdot))$ diminishes exponentially in $\mby f(\mbx)$, unless the gradient of the prediction function $\nabla_\theta f_\theta$ 
% TODO: how do we know $\nabla_\theta f_\theta$ isn't large? 
Note that the $(1- \sigma(\cdot))$ term is exponentially small in $\ftheta(\mbx)$ when the prediction ($\texttt{sgn}(\ftheta)$) is correct.
Then, as long as $\|\nabla_\theta f_\theta\|$ is not exponentially larger in magnitude than $|f_\theta|$, the gradients for the samples in the shortcut-\textit{misclassified} subset will drive the rest of training.
Here, a second race commences, between the noise, which will lead to overfitting, and the invariant features.
% 
If the model overfits to the shortcut-misclassified subset before it learns the invariant features, then gradients scale the coefficients to reduce the loss rather than learn new features.
However, the model continues to rely on the shortcut on the shortcut-classified subset from earlier.



In summary, when the shortcut wins the learning race with the invariant feature, models overfit to the remaining misclassified samples; as the shortcut feature continues to get used, we term this phenomenon \textit{preservation bias}.
The role of overparameterization here is twofold 1) the model's ability to overfit to the shortcut-classified subset faster than the invariant feature is learned and 2) allow the model to continue using the shortcut to correctly predict.
% 
TODO: rewrite; too quick, this even the right place?


Learning races and preservation bias provide one explanation for why \gls{erm} fails; but how do balancing methods or spectral decoupling help improve reliance on the invariant feature?
As we will discuss in detail next, both methods prevent the invariant feature from losing the learning races, thereby mitigating preservation bias.
% Balancing, via subsampling for example, reduces the maximum possible size of the shortcut-classified subset, which in turn increases magnitude of the gradients tha
% 
% 
% 
% Before we describe this prevention in more detail, 
To understand this better, we build intuition in a linear experiment.
% an image recognition perception task.

\subsection{Learning races and preservation bias in a linear perception task}


We first setup an intuitive linear data generating process where we demonstrate the intuition above.
Let $\ptr(\mby, \mbz, \mbx)$ correspond to the following data generating process: for a constant $B>1$, and $\cR$ as the uniform distribution over $\{-1,1\}$, and $\mbepsilon\sim \cN(0, \cI_{d-2})$ as isotropic gaussian noise in dimension $d-2$,
\[\mby \sim \cR, \mbz\in \{-1,1\}, \qquad  \ptr(\mbz = y \g \mby = y) = 0.9 \qquad \mbx = [\mbz, \nicefrac{\mby}{B}, \mbepsilon].\]


We generate a $1000$ samples and train a linear model (without an intercept term) for $100,000$ epochs with full gradient descent with $0.9$ momentum.
% We use to $d$ to vary the degree of overparameterization.
TODO: other details


\begin{figure}[t]
  \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{../figures/linear-preservation.png}
    \caption{
    As the dimension increases, the reliance on the invariant feature decreases.
    This occurs because as the dimension increases the gaussian noise features, memorization is easier and the invariant feature loses the learning race to this noise.
    }
    \label{fig:linear-preservation}
  \end{subfigure}%\
  \hspace{10pt}
  \begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{../figures/linear-preservation-balance.png}
    \caption{While subsampling does improve the relative reliance on the invariant feature over the shortcut, overfitting occurs due to the reduced size of the data.
    % In turn, held out accuracy is not perfect.
    % 
    This suggests the balancing does not help beyond a certain level of overparameterization.}
    \label{fig:linear-balancing}
  \end{subfigure}
  \caption{Learning races and preservation in the linear experiment. Accuracy and the ratio $r_p = \nicefrac{\that_y}{\that_z}$ in the linear experiment.
  In the accuracy plot, the solid lines are training accuracy, and the dashed lines are accuracy on a heldout dataset from the same distribution as the training data.
  The left image shows results via plain ERM while the right image compares to balancing.}
  \label{fig:linear-exps}
  \end{figure}

  We use a linear model $\that^\top \mbx$, and track the ratio of the weight on the invariant feature to the shortcut $r_p = \nicefrac{\that_y}{\that_z}$ as training progresses.
Working with $d=2$ and continuous-time gradient descent \citep{nagarajan2020understanding} prove that $r_p$ goes up as $\log t$ where $t$ is time.
% 
If this does happen, then eventually the invariant feature will outweigh the shortcut feature and the prediction should be perfect.
% 
However, for $B=10$, for $d\geq 300$ increases, $r_p$ plateaus to a constant; see \cref{fig:linear-exps}.
Further, the test accuracy also plateaus and does not converge 


\paragraph{Why and when does $r_p$ plateau to a constant? Why does it happen as $d$ increases?} 
To understand this phenomenon, let's look at the gradients of the loss w.r.t $\theta_z$ and $\theta_y$ 
\begin{align}
\nabla_{\that_z} \texttt{loss}= -  \frac{1}{n}\sum_i \left[1 - \sigma(\mby^i \ftheta(\mbx^i)) \right]\nabla_{\theta_z} \that^\top \mbx = -  \frac{1}{n}\sum_i \left[1 - \sigma(\mby^i \ftheta(\mbx^i)) \right] \mbz^i.  
\\ 
\nabla_{\that_y} \texttt{loss} = - \frac{1}{n} \sum_i \left[1 - \sigma(\mby^i \ftheta(\mbx^i)) \right]\nabla_{\theta_y} \that^\top \mbx = -  \frac{1}{n}\sum_i \left[1 - \sigma(\mby^i \ftheta(\mbx^i)) \right] \frac{\mby^i}{B}.
\end{align}
% 
The only difference between these two gradient terms is $\mbz^i$ and $\nicefrac{\mby^i}{B}$
The constant $B$ dampens the gradients 
and to match one step in $\that_z$, $\that_y$ needs $O(B^2)$ steps.
% In turn, increasing $B$ makes learning the invariant coefficient slower.
% 
%  
Thus, a large $B$ means the invariant feature loses the learning race with the shortcut feature $\mbz$.

A second ingredient determines whether the invariant feature gets picked up later in training: the dimension, which affects how noise is present in the covariates.
At $d=100$ the ratio $r_p$ continues to grow and the heldout accuracy is $100$, but for $d\geq 200$, the heldout accuracy is strictly less than $100\%$.
% 
The switch in behavior occurs at having enough parameters to memorize the shortcut-misclassified subset.
The subset where $\mby \not= \mbz$ is around a $100$ samples, because we have a $1000$ samples and the shortcut predicts the label $90\%$ of the time.
Then, even thought $d<n$, there are enough parameters to memorize a subset, which in turn induces a learning race between the invariant feature and the noise.
The larger the dimension, the faster overfitting occurs \footnote{
  For intuition here, note that for large dimension random gaussian vectors are orthogonal with high-probability in the gradients w.r.t $\that_\epsilon$ are
  % 
  $-\frac{1}{n}\sum_i \left[1 - \sigma(\mby^i \ftheta(\mbx^i)) \right] \mbepsilon^i,$
  which means one part of the linear prediction is $\propto \sum_i \mbepsilon_i^\top \mbepsilon_j \approx \|\mbepsilon_j\|^2$, which has an expected value of $O(d)$ (cite versheynin) that increases with dimension.
  So the magnitude of the gradients for $\that_\epsilon$ increase with dimension. 
TODO: sagawa say a similar orthogonal thing, be careful
  }
% 
meaning the training loss reaches $0$ faster and the gradients to learn the invariant feature are then cut off.
% 
This faster overfitting means the coefficient $\that_y$ see fewer gradient steps which leads to the ratio $r_p$ plateauing at a smaller value as dimension increases.


% So at $d>100$, the model is overparameterized with respectively to the
% As the dimension increases, more and more




\paragraph{Do balancing and spectral decoupling help? Why?}

In our linear perception task, both balancing and spectral decoupling do improve reliance on the invariant feature; see \cref{fig:linear-balancing}.

We consider balancing via subsampling.
By removing samples, subsampling makes the fraction of the subset where $\sho(\mbx^i)=\mby^i$ to be $0.5$; thus, the shortcut does not help predict the label better than chance.
As we observe in the (TODO), the heldout accuracy of the 
While this does mitigate the learning race between the shortcut and the nuisance, the race between overfitting and the invariant feature is relatively affected lesser.
To see why, note that the size of data after subsampling is typically only twice the size of the subset where $\mby^i \not= \mbz^i$ in the original dataset; thus, the invariant feature can only be twice as fast, which is insufficient to beat overfitting.


Next, spectral decoupling penalizes the value of $\ftheta$ by adding $\lambda \|\ftheta(\mbx^i)\|^2$ to the per-sample log loss.
Why?
Intuitively, the added penalty ensures that the logits do not get large, which in turn ensures that the $1- \sigma(\cdot)$ term does not go to $0$ and cut off gradients to the invariant feature from the shortcut-classified subset.
We observe that spectral improves over ERM both in heldout accuracy and in reliance on the perfect invariant feature; see \cref{fig:linear-sd}.
% 
\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
    \includegraphics[width=0.43\textwidth]{../figures/linear-preservation-SD.png}
  \end{center}
  \caption{Spectral decoupling on the linear example.}
  \label{fig:linear-sd}
  \vspace{-30pt}
\end{wrapfigure}



TODO: more detail
% In more detail, the per-sample gradient for $\that_y$ under spectral decoupling looks like 
% \[ - \left[1 - \sigma(\mby^i \ftheta(\mbx^i)) \right]\nabla_{\theta_y} \that^\top \mbx + \nabla_{\theta_y} \|\ftheta(\mbx^i)\|^2 = - \left[1 - \sigma(\mby^i \ftheta(\mbx^i)) \right] \frac{\mby^i}{B} + \ftheta(\mbx^i)\frac{\mby^i}{B}
% \]
% even thought the shortcut may be learned first, if the sigmoid


% TODO: figure
% - why does spectral decoupling help?

% - do methods like balancing and spectral decoupling always help?

% Balancing via subsampling however, does not show a significant improvement, even reducing the reliance on the invariant feature in certain cases.
% This however, is also explained by the learning race between the invariant and the noise features; the subset that remains after subsampling is only twice the maximum size of the shortcut-misclassified subset ($200$ in this case); at $d=300$, the whole dataset is overfit quickly.
% Methods like subsampling do prevent the learning race between the invariant and the shortcut features, but do not affect the race between the 
% In fact, this is what we show in \cref{fig:balancing}, balancing does help a little but ultimately does not ensure that the

\paragraph{If overfitting is the issue, does regularization help?}
% 
We experimented with $l2$-regularization and found that while it does reduce overfitting on the subset, it does not improve reliance on the invariant feature.

TODO: figure

To see why this is, note that the linear coefficient $\that_y$ needs to be $\Omega(B\that_z)$ to undo the mistakes of the shortcut.
This means that while heavy regularization can mitigate the learning race between overfitting and the invariant feature, it would also ensure reduces reliance on the invariant feature. 

\paragraph{Is this problem due to SGD? Does Adam help?}

% 
% In this experiment, the learning race was induced by scaling the invariant features.
Adam (cite) is an optimization method that scales the learning rate based on the past gradient magnitude.
Adam does in fact will update the learning rate by $O(B)$, because gradients for $\that_y$ are proportional to $1/B$.
This ensures Adam's updates are not dampened by $B$ as much as SGD; however, the coefficient $\that_y$ needs to reach a value of $B$ to cancel out the $\nicefrac{1}{B}$ in the covariates.
Further, Adam can also scale up the gradients for the noise features.
% 
In accordance to this intuition, we observe that Adam does improve over SGD when $d=100$ but makes the semantic feature lose the race faster for $d\geq 200$.

TODO: figure
% As we see in \cref{fig:adam-v-sgd}, Adam does improve the ratio over SGD for 

% A few questions arise from this explanation.



% 
% 


How do the observations on the linear experiment translate a more complex non-linear perception task?
For example, in SGD in the linear task, the rate at which a weight is learned is proportional to the magnitude of the variation of that feature in the covariates.
In deep neural networks however, other factors affect how fast a feature is picked up.
Next, we study learning races in an image recognition task.



\subsection{Learning races and preservation and an image recognition task}

We construct an image recognition with a perfect invariant feature (a CIFAR truck or car) and an imperfect shortcut (an MNIST image of a $0,1$) which only predicts the lable around $90\%$ of the time.
% 
% 
Our model consists of two identical convolutional resnets, one for each image, with their representations concatenated and fed through a linear layer.
% 
As convolutional networks can detect color even at initialization, the color feature is faster in the learning race than the CIFAR feature.

TODO: details about task setup

% Training to predict from the CIFAR-image alone achieves an AUC of $>0.95$; this is almost perfect prediction
% Together with the color being learned first, this suggests that preservation is occurring.

In this task, we intervene on the learning rate of the network that takes in the MNIST image and study the effect of setting it to be $0.1, 1, 10$ times the learning rate for the CIFAR feature; call this the \textit{multiplicative factor}.
The idea here is that the relative learning rate for the MNIST network changes the rate at which the MNIST features get picked up to be in the representation.
We then evaluate the reliance of the network on each image by randomizing the image and measuring the drop in AUC.

Reporting results for the best model (selected via validation loss over training), the overall AUC for each model is close to $0.95$.
But as the multiplicative factor increases from $0.1$ to $1$ to $10$, the reliance on the MNIST image goes up.$ to $1$ to $10$, the reliance on the MNIST image goes up.$ to $1$ to $10$, the reliance on the MNIST image goes up, as indicated by the MNIST-randomized AUC going down $0.70, 0.68, 0.66$.

TODO: run more seeds and average

\textit{What does this tell us?}
This increase in reliance on the MNIST image tells us that who wins the learning race between MNIST and the CIFAR images matters and affects which samples the model predicts using which images.



% ColorFalse_PREDboth_lrfac0.1
% Standard AUC:         0.955
% MNIST-Randomized AUC: 0.700
% CIFAR-Randomized AUC: 0.860
% Loss:                 0.269


% ColorFalse_PREDboth_lrfac1.0
% Standard AUC:         0.951
% MNIST-Randomized AUC: 0.677
% CIFAR-Randomized AUC: 0.882
% Loss:                 0.280


% ColorFalse_PREDboth_lrfac10
% Standard AUC:         0.948
% MNIST-Randomized AUC: 0.662
% CIFAR-Randomized AUC: 0.886
% Loss:                 0.284

\paragraph{Balancing and spectral decoupling TODO:}





\section{Discussion: Learning races, a unifying phenomenon}

- give answers to the questions we set out to answer

\subsection{The consequences of learning races and preservation}


- assume that preservation occurs, now point out that on the subset not predicted by the fast feature, flexible models can 1) overfit or 2) learn to predict using the perfect feature.

- if 1 occurs, ID generalization failure, but not 2.

- if 2 occurs or 1 occurs with the fast feature being the shortcut, then shortcut learning.





\paragraph{Overparameterization exacerbates preservation bias}


- as overparameterization increases, it should get easier to overfit to subsets or learn different features for different subsets, i.e.\ preservation should occur more often 


\paragraph{Summarizing the intuition for why preservation via balancing and preference-avoiding methods}


We identify the following directions can help avoid preservation

- slow down the fast feature to give time for the slow perfect feature to be learned.

A. (balancing) one way is to balance the data to reduce the dependence between the fast imperfect predictive feature and the label. 
    
    Further, balancing methods also ensure that because the fast feature can no longer predict well, overfitting requires memorizing a larger subset and gradients for the perfectly predictive feature are larger.

A2. Point out that this is what many shortcut-avoiding methods do (IMP: connect our work to methods that mitigate shortcut learning)

B. (not letting sigmoids peak) Another way are methods like spectral decoupling, which makes the sigmoid not peak which may maintain large gradients for the slow feature; we suggest a way to do this is to use likelihood parameterizations with heavy tails. (IMP: this is the only thing we can do if we don't know what to balance)

- regularize to ensure that a model cannot overfit on the incorrectly predicted (by the fast feature) subset. However, as we showed in the linear experiments, the amount of regularization required to prevent this subset-overfitting may restrict the model class too much.





\newpage
% \paragraph{Experiments}


% \begin{enumerate}
%     \item \textbf{(The existence of preservation bias)}; plot the fraction of samples that are shortcut-exploited at epoch 1 that continue to be shortcut exploited afterward.
%     This will be with randomly initialized neural networks.
    
    
%     \textbf{We expect} to see a large fraction of samples continue to be shortcut exploited after epoch 1.
    
    
%     \textbf{This supports} the existence of a preservation bias.
    
    
%     \item \textbf{(Overparameterization induces preservation bias)} : train resnets with increasing width on biased data and plot the distribution of largest per-sample change in shortcut-exploitation over epochs.
    
%     \textbf{We expect} to see models get more complex, more shortcut exploited samples continue to be shortcut exploited.
%     % We will compare which features the following models learn on a biased dataset: 1) model that is trained to predict the nuisance on balanced data and 2) model that is trained to predict the the label on balanced data.
%     % 
%     % For this experiment, we will use both pretrained and random models. 
%     % pretrained resnet50 model just like sagawa et al. (I will also run for rand init models but because they find it hard to learn the semantics, I have less faith these will work)

%     \textbf{We expect} that model 1 will have more shortcut exploited samples for the rest of training.
    
    
%     \textbf{This supports} preservation bias over other explanations for  which features are used by neural networks by the end of training.
    
    
%     \item \textbf{(Balancing experiments)}
    
%     We know balancing helps.
    
%     This supports why balancing methods help.
    
    
%     \item \textbf{(The role of pretraining in avoiding preservation bias)}
%     % 
%     Show first that preservation is much smaller in pretrained model by tracking the same thing from experiment 1.
%     % 
%     We point out a reason as pretraining leading to normalizing the rate of learning of the foreground and the background; this is evidenced (\textbf{we expect see}) by the switched training experiments and their difference from the plain ERM with pretrained model.
    
    
%     \textbf{This supports} the suggestion we have that normalizing the rates of learning for different features helps with OOD.
    
%     % \item \textbf{()}
    
%     \item \textbf{(optional, Adam vs. SGD experiments)}
    
% \end{enumerate}






% 1. Linear experiments
% 2. switched training experiment
% 3. more models min-max plots 


% TODO: all experiments done/to be done 


% Discussion


==> sections/related.tex <==

\section{Related work}

A large body of work tackles shortcut learning under different assumptions \citep{arjovsky2019invariant,krueger2020out,creager2021environment,veitch2021counterfactual,puli2022outofdistribution,heinze2017conditional,belinkov2017synthetic,jacobsen2018excessive}.
% Another line of work points out how biases in data can induce discriminatory predictions \citep{}.
On the other hand, work like \citep{yang2019fine,ronen2019convergence,jo2017measuring,baker2018deep,saxe2013exact,gidel2019implicit,advani2020high} focuses on understanding what neural networks learn in idealized settings.
The closest to our paper are two lines of work that study how feature learning occurs in neural networks and how it affects modeling with and without shortcuts.

The first deals with understanding which features neural networks prefer to learn first: \citep{hermann2020shapes,shah2020pitfalls,nakkiran2019sgd,scimeca2021shortcut}.
At a high-level, these works focus on biases that appear due to neural architectures interacting with gradient descent.
We, on the other hand, point out how gradient-based training of flexible models leads to data wastage, which prevents networks from learning even perfectly predictive features.

\cite{hermann2020shapes} empirically demonstrate that when two features (shape and texture in images) predict perfectly, features that are linearly classifiable at initialization are preferred; 
\citet{scimeca2021shortcut} make similar observations for different synthetic datasets and empirically connect loss landscapes of neural networks and why some features are easier to learn.
% 
\citet{hermann2020shapes} also show that a linearly decodable but weaker predictive feature is preferred over a non-linear more predictive feature.
This is similar to \citet{shah2020pitfalls}, who study simplicity bias \citep{valle2018deep} and show that, for a certain simulated dataset, neural networks provably approximate the simpler linear function at one epoch.
% 
In a closer relation to our paper, \citep{shah2020pitfalls} show that even when the simpler(linear) feature is less predictive ($95\%$) than the complex (non-linear) features, the simpler one is used.


Beyond the linear vs. non-linear dichotomy it is unclear what simple features mean; both \citep{hermann2020shapes} and \citep{shah2020pitfalls} rely on this dichotomy as evidence of neural networks preferring simpler features.
% 
% 
Second, simplicity bias alone is an incomplete explanation of why other more complex functions are not learned later in training; \citep{nakkiran2019sgd} suggest SGD on neural networks learns functions of increasing complexity.
While simplicity bias explains quicker learning of one feature, our mechanism explains why more complex functions may not be learned after.
Unlike \citep{hermann2020shapes,scimeca2021shortcut}, we give an intuitive linear  where models end up relying on imperfect features even when there is a perfectly predictive feature.


The second line of work aims to understand the biases in gradient-based dynamics.
Using similar intuition to our work, 
\citet{pezeshki2021gradient} hypothesize when one feature is learned first, other features are gradient-starved.
%We point out explicitly how gradients from correctly and confidently classified samples vanish.
% version of this phenomenon where we identify how gradients from certain examples disappear during training.
% 
% 
% 
% rr: one line here that could help is that we say the gradient from examples disappears
% apm: DONE
%In contrast to \citet{pezeshki2021gradient} who define the singular vectors of the neural tangent random feature (NTRF) matrix, in the idealized NTK regime, as the features, we focus on the features in the covariates (e.g. foreground vs. background).
Further, to derive theory, \citet{pezeshki2021gradient} define features using the neural tangent random feature (NTRF) matrix and make restrictive assumptions about each feature appearing in single samples.
Due to such restrictions, the theory in \citet{pezeshki2021gradient} cannot explain why confidence controlling methods (like spectral decoupling) and balancing methods work on common OOD perception tasks where perfect semantic features are shared across all samples.
% It is unclear when the NTRF features match image features, and whether the NTK is stable enough (a requirement for NTK-based theory to hold) in experiments that run for $100$s of epochs.
%As \citet{pezeshki2021gradient} focus on NTK features and restrict how features appear in data points, their theory does not explain why confidence controlling methods (like spectral decoupling) and balancing methods work on common OOD tasks where semantic features are shared across samples.




\citet{nagarajan2020understanding} consider a case where the semantic feature perfectly predicts the label (like in perception tasks) while the shortcut is imperfect; they show that vanilla gradient descent is slow to learn to rely on the semantic feature.
Their setting does not point out the role of overparameterization (except for relying on an "increasing norms" property that is empirically observed for overparameterized models); accordingly, we point out a dimension-dependent behavior of the reliance on the shortcut feature in the linear model.
%
\citep{sagawa2020investigation} point out overparameterized models are more prone to spurious correlations because they can memorize the subset where the shortcut misclassifies (the minority group).
In the theory in \citet{sagawa2020investigation}, there is no perfectly predictive feature and the shortcut (the shortcut) has a much stronger relationship with the label than the semantic feature; they focus on the max-margin solution which even balancing may not help reach without additional regularization.
While \citet{khani2021removing} have both perfect features and overparameterization, they investigate a different conclusion: they investigate when removing the shortcut from the covariates can hurt performance.
They study a linear data generating process where the label and the shortcut can affect the same features in the covariates.


To validate the data-wastage mechanism on common OOD tasks, we control confidence as a way to intervene in learning to reduce data wastage.
To this end, we show that using architectural restrictions and loss-parameterizations to control confidence improve semantic reliance on waterbirds vs. landbirds and celeba \citep{sagawa2019distributionally}.
The confidence-controlling techniques we use are related to work like 
\citep{liu2017sphereface,cao2019learning,kini2021label} although their motivations are not to control confidence;
these works normalize representations or the last linear layers and linearly transform the logits which is shown to learn models with better margins under label imbalance.
%hese works which either modify the cross-entropy loss or normalize representations or the last linear layer to improve modeling in the presence of label imbalance and fairness across groups.
%While \cite{liu2017sphereface} normalize the last linear layer to learn features that are better discriminated by angular distance between representations, 
%\cite{cao2019learning} normalize both the representation and the last linear layer to make it easy to enforce class-dependent margins in cross-entropy to improve learning under label-imbalance; in contrast, we use the normalization to control confidence.
%Unlike \cite{kini2021label} who transform logits as $ m_y w^\top r(\mbx_i) + a_y$, we raise to a fractional power $\left(w^\top r(\mbx_i)\right)^{1/3}$ to reduce the rate of confidence peaking.
%In contrast, \cite{kini2021label} improve margins in the presence of label-imbalance by using class-dependent additive and \textit{multiplicative} adjustments in cross entropy loss where the logits are transformed as $ m_y w^\top r(\mbx_i) + a_y$.
%\cite{liu2017sphereface} reason about features that are better discriminated by angular distance between representations (rather than euclidean distance) and propose the angular softmax loss where the logit (for binary classification) is  given as $\nicefrac{w^\top}{\|w\|}r(\mbx_i)$.
%\cite{cao2019learning} enforce class-dependent margins in cross-entropy to improve learning under label-imbalance; to be able to better tune said margin, they normalize the representation and produce logits as $\nicefrac{w^\top}{\|w\|}\nicefrac{r(\mbx_i)}{\|r(\mbx_i)\|}$, restricting them range $[-1,1]$.
%\cite{kini2021label} propose to use class-dependent additive and \textit{multiplicative} adjustments in cross entropy loss where the logits are transformed as $ m_y w^\top r(\mbx_i) + a_y$.
Note that these works make architectural or loss-adjustments that either prevent confidence of prediction from peaking quickly or bound the confidence explicitly.



==> sections/sec3_old.tex <==
\subsection{Vanishing data.}
\hl{TODO: move a bunch of the math in this subsection to the appendix; only main points should remain here.}

% 1. If sample have low-loss they contribute less to the gradient. (math and plot)
% apm: depend = vary with a feature


% Briefly, the vanishing-data mechanism is that models depend on shortcuts to reduce loss which in turn leads training to fit to noise on the well

% \hline{}


% Vanishing data mechanism definition (needs math)


%  - Loss can be driven down to low levels for individual data points, these data points can vanish from learning in a flexible model
%   (math like a gradient computation to show that the loss is small these examples don't provide gradients to anything anymore)
% larger the norm of the gradient for the first-layer weights that touch noise, and the smaller the gradients for the stable feature.
% 

% % apm: bad writing
% We begin by looking at how when a subset of samples has small enough log-loss, the optimization makes model fit to noise on the high-loss samples over the perfect feature.
% We call the data with the small loss \textit{vanishing} due to it's diminishing role in learning the perfect feature.

% We now provide a simplified analysis of a two-layer network trained on our synthetic example to how low-loss samples affect optimization on the high-loss subset.
% Specifically, we show how gradients for the first layer of the neural network propagate noise into the network, which in turn can lead the model to overfit to the high-loss subset.

In this section, now describe the concept of vanishing data. Data has vanished if the \hl{todo}.

To explain this phenomenon in detail, we analyze a simple example of a two-layer network trained on data generated as described in the previous section. Specifically, we show how \hl{todo}. Then, we show how gradients for the first layer of the neural network propagate noise into the network, which in turn can lead the model to overfit to the high-loss subset.

\paragraph{Preliminaries on gradients, confidence, and loss.}
To first understand how low-loss implies gradients are weighed down, consider the gradient of the log-loss $\ell(\ftheta(\mbx), \mby) = \log \left[1 + \exp(-\mby \ftheta(\mbx))\right]$ w.r.t $\theta$:
\begin{align}
\label{eq:grad-logloss}
\begin{split}
    \nabla_\theta \ell(\ftheta(\mbx), \mby)) & = -\frac{\exp(-\mby \ftheta(\mbx))}{1 + \exp(-\mby \ftheta(\mbx))} \mby \nabla_\theta f_\theta(\mbx) 
    \\
            & = - \frac{\mby \nabla_\theta f_\theta(\mbx)}{1 + \exp(\mby \ftheta(\mbx))}.
\end{split}
\end{align}
% 
% 
%
% 
% The magnitude of the gradient from each sample is modulated by how confidently correct the prediction on that sample is; as $\mby \ftheta(\mbx)$ gets larger, $\nabla_\theta f_\theta(\mbx)$ gets smaller.
% 
% 
% 
% For loss to get small, $|f(\mbx)|$ needs to increase while $\mby=\texttt{sgn}(\ftheta)$, i.e. the confidence of prediction $\sigma(|\ftheta(\mbx)|)$ should be high.
% Then the term in the denominator, $1 + \exp(\mby \ftheta(\mbx))$, is exponentially large in $|\ftheta(\mbx)|$.
% When $\|\nabla_\theta f_\theta\|$ is bounded the gradients for the samples with small loss will be weighed down exponentially in $|f_\theta(\mbx)|$.


% \paragraph{Vanishing data can propagate noise in models.}



\hl{TODO: I say both subsets classified correctly but one subset with lower confidence $1-\gamma$; this is what happens in the training data anyway in the experiments I think.}

Denote with $S$ the subset with correctly classified samples with confidence $1 - \epsilon$. Let its complement $S^c$ contain also correctly classified samples with lower confidence $1 - \gamma$, where $\gamma > \epsilon$.
First, for correctly classified samples, $\mby\ftheta(\mbx) = |\ftheta(\mbx)|$ and for misclassified samples $\mby\ftheta(\mbx) = - |\ftheta(\mbx)|$.
For the subsets, the denominator in \cref{eq:grad-logloss} is
\begin{align}
\label{eq:den-control}
\begin{split}
\text{in } S\quad 1 + \exp(|f(\mbx)|) = \frac{1}{\epsilon}.
\\
\text{in } S^c\quad 1 + \exp(|f(\mbx)|) = \frac{1}{\gamma}.
\end{split}
\end{align}
% 
% 
% - small loss samples removed from training
% 



\paragraph{Splitting the total gradient}
Let $\theta = [w_2, w]$ be the neural network parameters.
With $r(a) = \max(a,0)$ as the \texttt{relu} function, let the model $\ftheta(\mbx) = w_2^\top r(w^\top \mbx).$
The gradient of the loss with respect to the first layer of the neural network $w$ is as follows:
%
% 
\begin{align}
\label{eq:total-grad-vanishing}
\begin{split}
&\Delta_{\Dtr} = \sum_{i\in \Dtr } \nabla_w \log(1 + \exp(\mby^i\ftheta(\mbx^i)))
\\
   = & \sum_{i\in S}\nabla_w \log(1 + \exp(\mby^i\ftheta(\mbx^i))) 
   \\
    & \quad + \sum_{i\in S^c}\nabla_w \log(1 + \exp(\mby^i\ftheta(\mbx^i)))
\\
    = & - \sum_{i\in S} \frac{ w_2^\top 1[w^\top\mbx^i > 0] \mby^i \mbx^i}{1 + \exp(|\ftheta(\mbx^i))|} - \sum_{i\in S^c} \frac{ w_2^\top 1[w^\top\mbx^i > 0] \mby^i\mbx^i}{1 + \exp(|\ftheta(\mbx^i))|},
\\
    = & - \Delta_S + - \Delta_{S^c},
\end{split}
\end{align}
where $\Delta_S, \Delta_{S^c}$ denote gradient-steps on $S$ and $S^c$.


\paragraph{Gradients on $S$ and its contribution to learning the perfect feature.}
% apm: justifidable adverbs
To achieve high confidence, neural network representations must have large inner product with the linear layer; so, for samples in $S$, we assume ${ |w_2^\top 1[w^\top\mbx^i > 0] \mbx}| \leq |w_2^\top r(w^\top\mbx^i)| = |\ftheta(\mbx)|$, where $w, w_2$ are both vectors of the same dimension as $\mbx$.
Note that for the correctly classified samples in $S$, the denominator is $1 + \exp(|\ftheta(\mbx)|)$ which is exponentially large in $|w_2^\top r(w^\top\mbx^i)|$.
% Thus, $ |w_2^\top 1[w^\top\mbx^i > 0] | \leq  $
Then, using \cref{eq:den-control}., the gradients in $\Delta_S$ in \cref{eq:total-grad-vanishing} are weighted down by a term bounded by $c \epsilon$ where $c << {1}{\epsilon}$.
The second coordinate $\mbx^i_2 = \frac{\mby^i}{10}$.
Then, the gradient update to $w_2$, the coordinate of $w$ that touches $\mbx_2$, from $\Delta_S$ is approximately $\frac{c|S|\epsilon}{10}$.
% Denote by $\Delta_{2$ the
% So instead, we focus on where the 
% Thus, the gradient

% Thus, we approximate the first term in \cref{eq:total-grad-vanishing} with $\epsilon \mby^i\mbx^i$ and rewrite it as
% \begin{align}
% \label{eq:small-loss-grad}
% \begin{split}
% - {\epsilon}\left[\sum_{i\in S, \mby^i=1} \mbx^i 
%   - \sum_{i\in S^c, \mby^i=-1} \mbx^i\right]
% \end{split}
% \end{align}
% 
% As the confidence, $\epsilon$, this term vanishes from the, then samples from $S^c$

\paragraph{Gradient on $S^c$.}

Let's look at the gradient samples in $ S^c $ now, splitting between different labels.
Recalling from \cref{eq:den-control} that $1 + \exp(|\ftheta(\mbx^i))| = \nicefrac{1}{\gamma}$, and assuming that 
$w_2^\top 1[w^\top\mbx^i > 0] =\alpha$ across the high-loss samples,
\begin{align}
\label{eq:total-grad-split}
\begin{split}
& \Delta_{S^c} = \sum_{i\in S^c} \frac{ w_2^\top 1[w^\top\mbx^i > 0] \mby^i\mbx^i}{1 + \exp(-|\ftheta(\mbx^i))|} = 
% \\
%     & = \frac{1}{\gamma}\left[ \sum_{i\in S^c, \mby^i=1}w_2^\top 1[w^\top\mbx^i > 0] \mbx^i \right.
%     \\
%         & \quad - \left.\sum_{i\in S^c, \mby^i=-1}w_2^\top 1[w^\top\mbx^i > 0] \mbx^i\right]
% \\
    % & = 
   -  {\alpha\gamma}\sum_{i\in S^c} \mby_i\mbx^i 
    % \mby^i=1} \mbx^i 
%   - \sum_{i\in S^c, \mby^i=-1} \mbx^i\right]
\end{split}
\end{align}

\paragraph{How noise propagates through the first layer?}

Next, we look at how these gradients differ for differ features.
Denote $\Delta_2$ as $\Delta_{S^c}$'s coordinate that corresponds to the weights associated with the perfect feature $\mbx_2$, and $\Delta_n$ as the gradient that corresponds to weights associated with the noise features $\mbx_{3\cdots d}$.
Next, we discuss as the number of samples in $S^c$ decrease, $\frac{\|\Delta_n\|}{|\Delta_2|}$ increases.
This means that as $S^c$ decreases in size, optimization makes the first layer $w$ depend more on noise dimensions in $\mbx$, i.e noise propagates in the first layer.


First, we express the ratio as $\frac{\|\Delta_n\|}{|\Delta_2|} = \frac{\|\Delta_n/|S^c|\|}{|\Delta_2/|S^c|\|}$.
Recalling that $\mbx_2 = \nicefrac{\mby}{10}$ and that $\mby^2 = 1$,
shows that $\frac{\Delta_2}{|S^c|}$ does not vary with the size of $S^c$:
\[\left|\frac{\Delta_2}{|S^c|}\right| = \frac{1}{|S^c|}\left|\alpha\gamma \sum_{i\in S^c} \mby^i \frac{\mby^i}{10}\right| =  \frac{|\alpha\gamma|}{10} .\]

Next, note that as $\mby\indep \mbdelta$, the $\mby^i \mbdelta^i$ is distributed identically to $\mbdelta$ (an isotropic Gaussian).
Thus the norm of $\Delta_n$ is distributed as a constant times the norm of a mean of $|S^c|$ gaussian vectors, denoted $\bar{\mbdelta^i}_{i\in S^c}$
\[\frac{\|\Delta_n\|}{|S^c|} = \left\|\frac{1}{|S^c|}\alpha\gamma\sum_{i\in S^c} \mby^i \mbdelta^i \right\| =\alpha\gamma \|\bar{\mbdelta^i}_{i\in S^c}\|.\]
The probability that a $d$-dimensional Gaussian vector with unit-variance coordinate has norm outside $[(1-u)\sqrt{d},(1+u)\sqrt{d}]$ is exponentially small in $du$ \citep{vershynin2018high}.
Noting that $\sqrt{|S^c|}\nicefrac{\Delta_n}{|S^c|}$ is a Gaussian vector with unit-variance coordinates.
Thus, with high probability $\nicefrac{\|\Delta_n\|}{|S^c|}\propto \sqrt{\nicefrac{d}{|S^c|}}$.
Thus, as $|S^c|$ decreases, $\nicefrac{\|\Delta_n\|}{|S^c|}$ increases and therefore $\nicefrac{\|\Delta_n\|}{|\Delta_2|} $ increases


(TODO: the following title is for us, should remove it after summarizing the big section)
\paragraph{Putting it all together.}
Note that overall contribution to learning the perfect feature is $\frac{1}{10}\left(|S^c|\alpha\gamma + c|S|\epsilon\right)$.
When loss on $S$ is sufficiently small to have $c\epsilon < \alpha\gamma$, this quantity gets smaller when $S$ increases, that is $S^c$ decreases.
At the same time, the relative contribution of the noise from $S^c$ to the gradients in first layer increases compared to the perfect feature.
Summarizing, for a large $S$, gradient steps the first layer of the network fits $S^c$ more with noise and less with the perfect feature.
This gives us a mechanism to explain how shortcut learning occurs in the presence of a perfect stable feature, as we discuss next.


TODO: is there a plot here to disarm any of the "this is too weird an analysis."

TODO: should we talk about what happens when $S$ is large? about noise not being able to fit? Could be an aside.



\subsection{The vanishing data mechanism.}

% The previous subsection shows that the fewer samples have high loss, the larger the more noise propagates through the first layer and can become available for the layer layers to fit to.


\hl{TODO: make sure the following comes across:}

When a model depends on the shortcut, the loss on the shortcut group ($\mby=\mbz$) is small and the minority group $(\mby\neq\mbz)$ is big.
By the vanishing data mechanism, as the shortcut group gets big, the models fits more to the noise from $S^c$ than the perfect feature.
This means for a large enough shortcut group, model can fits to the shortcut and the noise to classify the whole dataset correctly.


\hl{TODO: erm-figure explanation, per-group losses}

Show from the plots that this actually happens.


1. Look at the test loss on the minority group, see that it does not go down as fast as the majority.

2. see minority in train vs. test, see model fits to noise.


% 1*. If fewer samples have high loss, the larger the norm of the gradient for the first-layer weights that touch noise, and the smaller the gradients for the stable feature.


